The Signed Two-Space Proximity Model for Learning Representations in Protein-Protein Interaction Networks

Accurately predicting complex protein-protein interactions (PPIs) is crucial for decoding biological processes, from cellular functioning to disease mechanisms. However, experimental methods for determining PPIs are computationally expensive. Thus, attention has been recently drawn to machine learning approaches. Furthermore, insufficient effort has been made toward analyzing signed PPI networks, which capture both activating (positive) and inhibitory (negative) interactions. To accurately represent biological relationships, we present the Signed Two-Space Proximity Model (S2-SPM) for signed PPI networks, which explicitly incorporates both types of interactions, reflecting the complex regulatory mechanisms within biological systems. This is achieved by leveraging two independent latent spaces to differentiate between positive and negative interactions while representing protein similarity through proximity in these spaces. Our approach also enables the identification of archetypes representing extreme protein profiles. S2-SPM's superior performance in predicting the presence and sign of interactions in SPPI networks is demonstrated in link prediction tasks against relevant baseline methods. Additionally, the biological prevalence of the identified archetypes is confirmed by an enrichment analysis of Gene Ontology (GO) terms, which reveals that distinct biological tasks are associated with archetypal groups formed by both interactions. This study is also validated regarding statistical significance and sensitivity analysis, providing insights into the functional roles of different interaction types. Finally, the robustness and consistency of the extracted archetype structures are confirmed using the Bayesian Normalized Mutual Information (BNMI) metric, proving the model's reliability in capturing meaningful SPPI patterns.

==> enrichment_sup.tex <==
To[a] elucidate the biological relevance of the identified clusters, we performed [ ] on the proteins of each cluster. We found the clusters to be enriched for proteins related to distinct biological processes. For instance, cluster 4 captures the processes of antiviral immune response. More specifically, it captures positive regulation of Inteferon-apha which is a type of Interfore I and is produced in response to viral infection mainly by immune cells involved in innate immune response (https://www.ncbi.nlm.nih.gov/pmc/articles/PMC4084561/, https://www.nature.com/articles/nri888). In addition, cluster 7 captures key processes and components integral to mitosis, the last phase of the cell cycle, a type of cell division in eukaryotes essential for growth, development, and repair (https://www.sciencedirect.com/science/article/pii/S1084952121001658?via%3Dihub review 2021). In particular, it focuses on the dynamics of microtubules, activity of myosin phosphatase and
MAPK cascade. Microtubules, one of the principal components of cell cytoskeleton, form the mitotic spindle, a macromolecular machine which through direct interaction with mitotic chromosomes ensures precise chromosome segregation during mitosis (https://www.ncbi.nlm.nih.gov/books/NBK9932/). https://pubmed.ncbi.nlm.nih.gov/12142285/ 2002,https://pubmed.ncbi.nlm.nih.gov/18275887/ 2008,https ://www.nature.com/articles/nrm.2016.162 2017 review, https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6756986/). Furthermore, the MAPK (Mitogen-Activated Protein Kinase) pathway comprises a cascade of protein kinases that serve as crucial regulatory points in cell proliferation. This pathway includes the ERK (Extracellular signal-Regulated Kinase) subgroup, which plays a key role in activating mitosis (https://www.nature.com/articles/7290105/figures/1). The activity of myosin phosphatase has also been associated with the process of mitosis (https://www.sciencedirect.com/science/article/pii/S0167488918302337). Other clusters identified were found to be associated with multiple biological processes among which can be outlined: cell adhesion, migration, development (cluster 0), G protein-coupled receptor (GPCR) signaling pathways and their effects on neuronal functions and interactions (cluster 1), cellular communication and the extracellular environment (cluster 2), signaling pathways involving GTPases (cluster 3), [cluster 5 is too scarce I believe]. Cluster 6 is more complex in comparison to other clusters derived from negative regulation and encompasses a range of cellular processes and structures primarily associated with autophagy, cell division and DNA damage. Similarly to cluster 6, all clusters identified through positive regulation are more complex and are associated with a range of biological processes and components.
H.sapiens negative regulation clusters
Summary of the clusters
Cluster 0: associated with processes of development, epithelial-mesenchymal transition (EMT)
Cluster 1: signal tranmission
Cluster 2: cell communication associated with extracellular matrix
Cluster 3: signal tranduction
Cluster 4: P:defense response to virus; P:innate immune response; mRNA binding; P:positive regulation of interferon-alpha production; P:positive regulation of type I interferon production
describe porcesses associated with antiviral immune response: https://www.ncbi.nlm.nih.gov/pmc/articles/PMC4084561/ on Regulation of type I interferon responses
This cluster is associated with immune response, specifically, antiviral
              
 Intefreron-apha is a type of Interfore I
“Type I or 'viral' IFNs include IFN-α, IFN-β, IFN-ω and IFN-τ”
https://www.nature.com/articles/nri888
So in general, it describes positive regulation of type I interferon production, more specifically Interferon-alpha, which is known to mount antiviral responses.
Cluster 5: processes associated with gene expression and metabolism?
Cluster 6: It is more complicated to describe, a mixture of autophagy and Mitochondrial Components, Cell Division and Chromosome Organization, Apoptosis and DNA Damage Response, Protein and Complex Interactions
Cluster 7: mytotic cell cycle
This cluster seems to capture processes associated with cell proliferation, more specifically mitotic cell cycle. It includes microtubules which are cytoskeleton components playing an essential role in cell division as well as
P:cell division; structural constituent of cytoskeleton; P:mitotic cell cycle; C:mitotic spindle; C:microtubule cytoskeleton; C:microtubule; P:microtubule cytoskeleton organization; myosin phosphatase activity; P:MAPK cascade
cell+division+structural+constituent of cytoskeleton+mitotic cell cycle+mitotic spindle+microtubule cytoskeleton+microtubule+microtubule cytoskeleton organization+myosin phosphatase activity+MAPK cascade
microtubule and mitosis
29. Bahmanyar S, Nelson WJ, Barth AI. Role of APC and its binding partners in regulating microtubules in mitosis. Adv Exp Med Biol 2009; 656:65–74 [PMC free article] [PubMed] [Google Scholar]
30. Sarangapani KK, Asbury CL. Catch and release: how do kinetochores hook the right microtubules during mitosis? Trends Genet 2014; 30:150–9 [PMC free article] [PubMed] [Google Scholar]
31. Tanaka K. Dynamic regulation of kinetochore-microtubule interaction during mitosis. J Biochem 2012; 152:415–24 [PubMed] [Google Scholar]
32. Tanaka K. Regulatory mechanisms of kinetochore-microtubule interaction in mitosis. Cell Mol Life Sci 2013; 70:559–79 [PubMed] [Google Scholar]
Mitotic spindle and microtubule
https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6756986/
                
 MAPK in proliferation
https://www.nature.com/articles/7290105 https://www.ncbi.nlm.nih.gov/pmc/articles/PMC10605237/ review Myosine phosphatase
https://pubmed.ncbi.nlm.nih.gov/11942620/ review https://www.sciencedirect.com/science/article/pii/S0167488918302337
To elucidate the biological relevance of the identified clusters, we performed [ ] on the proteins of each cluster. We found the clusters to be enriched for proteins related to distinct biological processes. For instance, cluster 4 captures the processes of antiviral immune response. More specifically, it captures positive regulation of Inteferon-apha which is a type of Interfore I and is produced in response to viral infection mainly by immune cells involved in innate immune response (https://www.ncbi.nlm.nih.gov/pmc/articles/PMC4084561/, https://www.nature.com/articles/nri888). In addition, cluster 7 captures key processes and components integral to mitosis, the last phase of the cell cycle, a type of cell division in eukaryotes essential for growth, development, and repair (https://www.sciencedirect.com/science/article/pii/S1084952121001658?via%3Dihub review 2021). 

In particular, it focuses on the dynamics of microtubules, activity of myosin phosphatase and MAPK cascade. Microtubules, one of the principal components of cell cytoskeleton, form the mitotic spindle, a macromolecular machine which through direct interaction with mitotic chromosomes ensures precise chromosome segregation during mitosis (https://www.ncbi.nlm.nih.gov/books/NBK9932/). https://pubmed.ncbi.nlm.nih.gov/12142285/ 2002,https://pubmed.ncbi.nlm.nih.gov/18275887/ 2008,https ://www.nature.com/articles/nrm.2016.162 2017 review, https://www.ncbi.nlm.nih.gov/pmc/articles/PMC6756986/). Furthermore, the MAPK (Mitogen-Activated Protein Kinase) pathway comprises a cascade of protein kinases that serve as crucial regulatory points in cell proliferation. This pathway includes the ERK (Extracellular signal-Regulated Kinase) subgroup, which plays a key role in activating mitosis (https://www.nature.com/articles/7290105/figures/1). The activity of myosin phosphatase has also been associated with the process of mitosis (https://www.sciencedirect.com/science/article/pii/S0167488918302337). Other clusters identified were found to be associated with multiple biological processes among which can be outlined: cell adhesion, migration, development (cluster 0), G protein-coupled receptor (GPCR) signaling pathways and their effects on neuronal functions and interactions (cluster 1), cellular communication and the extracellular environment (cluster 2), signaling pathways involving GTPases (cluster 3), [cluster 5 is too scarce I believe]. Cluster 6 is more complex in comparison to other clusters derived from negative regulation and encompasses a range of cellular processes and structures primarily associated with autophagy, cell
division and DNA damage. 






Similarly to cluster 6, all clusters identified through positive regulation are more complex and are associated with a range of biological processes and components.







              
Comment: Multiple processes with positive regulation, does it make sense? H.sapiens negative regulation clusters
Cluster 0: a wide array of processes that are positively regulated, especially focusing on differentiation, signalling pathways, transcription regulation, and development across multiple systems.
Cluster 1: ...
:
Cluster 6: describe the process of ubiquitination
Cluster 7: development and immune response? possibly the development of the immune system during differentiation?

==> introduction.tex <==
\section{Introduction}

%Analyzing and predicting complex relationships in biological networks is of paramount importance for drug discovery, personalized medicine, and combating diseases effectively. 
Proteins, as the building blocks of the cell, interact with each other due to biochemical events in order to carry out various cellular functions \citep{legrain2001protein}. 
%Interactions between proteins form complex networks among other biological pathways, known as the interactome \citep{cusick2005interactome} and regulate various molecular mechanisms within biological systems.
%Capturing protein-protein interactions (PPIs) is thus fundamental for decoding cellular processes that importantly encrypt disease mechanisms. 
Interactions between proteins form complex networks within biological pathways, collectively known as the interactome \citep{cusick2005interactome}, which regulate various molecular mechanisms within biological systems. Capturing protein-protein interactions (PPIs) is therefore fundamental for decoding cellular processes, crucially implicated in disease mechanisms \citep{rual2005towards}.
However, experimental methods for the determination of PPIs, such as yeast two-hybrid systems \citep{ito2001comprehensive}, mass spectrometry \citep{gavin2002functional}, and protein chips \citep{zhu2001global}, among others, are often characterized as computationally expensive, time-consuming and insufficient \citep{han2005effect}. 
%Similarly in pharmacology, discovering how drugs interact with each other plays a crucial role in optimizing therapeutic regimens, mitigating adverse effects, and minimizing adverse drug-drug interactions (DDIs).
%DDIs can lead to unpredictable outcomes, ranging from diminished efficacy to severe toxicity, posing significant challenges in clinical practice. 
%Traditional methods for assessing DDIs which rely on labor-intensive experimentation and clinical observations are also rather restrictive.
%To overcome the experimental limitations in capturing relationships in PPI networks, advanced computational techniques, that often rely on machine learning have recently become very promising. 
%These techniques are often experimentally proven to extract valuable information from available biological networks and generalize the prediction of potential relationships with great accuracy on unseen data, while remaining computationally efficient. 
To overcome the experimental limitations in capturing relationships in PPI networks, advanced computational techniques, often relying on machine learning, can offer a viable solution.

%Sequence-based methods for predicting PPIs focus on capturing relationships between complex features extracted from the underlying amino-acid sequences. Such computational methods have been primarily driven by machine learning \citep{bock2001predicting} and more recently deep learning methods \citep{noisy_ppi3}. Dominant machine learning approaches are built upon measures such as autocovariance (AC) \citep{guo2008using}, distance similarities \citep{zaki2009protein}, and methods based on support vector machines (SVMs) \citep{guo2010pred_ppi}, k-Nearest Neighbor (KNN), decision trees \citep{chen2005prediction} and hidden Markov models (HMMs). The application of deep learning methods, that are tailored to capturing intricate non-linear relationships on high-dimensional input features, has also gathered great attention for predicting PPIs, built upon various neural network architectures \citep{zhang2019protein,zeng2020protein}, such as convolutional and recurrent ones.





Protein-protein interaction networks can be modeled to be signed instead of just indicating the presence or absence of interactions. 
This representation can capture both activating (positive) and inhibitory (negative) interactions. 
The signed formulation allows a natural representation of biological relationships, which is crucial for the effective modeling of complex regulatory mechanisms within biological systems \citep{pritykin2013simple}.
Several representation learning methods for signed graphs have been proposed over the years for tasks spanning from community detection \citep{signed_com1,signed_com2} to link prediction \citep{slink1}, focusing mostly on social network applications.
Representative methods in this field have been built upon the psychological-based concept of balance theory \citep{cartwright1956structural} and random walks \citep{perozzi2014deepwalk} to capture interactions.
Specifically, \textsc{SIDE} \citep{side} and \textsc{POLE} \citep{pole} models focus on extracting random walks for signed graphs while capturing pair-wise signs based on balance theory.
In such terms, neural networks have also been employed to capture signed interactions.
Notable methods include \textsc{SiGNET} \citep{signet} that combines multi-layer perceptrons with balance theory \citep{signet} and \textsc{SLF} \citep{slf} that introduces multiple latent factors that model additional types of interactions.
%Graph neural networks, \ie a family of neural networks that operate on graph structure data, have also been applied to capturing signed interactions on networks.
Built upon graph neural networks (GNNs), \textsc{SiGAT} \citep{sigat} combines common theories for signed networks with graph attention networks.
On the other hand, a recent approach, \textsc{SPMF} \citep{SPMF}, extracts node representations using low-rank matrix approximation to better encode multi-order signed proximity.
%SLIM, POLE, SLF, SIGAT, SDGNN, SPMF are used as baselines -> maybe remove some from the rest (SIDE, SiGNET)

Unsupervised learning and clustering techniques are fundamental for uncovering hidden patterns and structures in protein-protein networks \citep{pro_clus}. Originally, Archetypal Analysis (AA) \citep{cutler1994a,5589222} was introduced for analyzing observational data that are constrained to a $K$-dimensional polytope, in which each observation can be expressed as the convex combination of the polytope's corners, with the latter forming the archetypes.
AA has been extended to various domains such as computer vision \citep{Chen_2014_CVPR}, and population genetics \citep{Gimbernat-Mayol2021.11.28.470296}, while many studies have focused on the scalability and robustness of relevant methods \citep{EUGSTER20111215,AA_prac}.
Archetypal Analysis has been recently extended to relational data \citep{SLIM,SGAAE}, with applications to analyzing signed social networks under the Skellam distribution \citep{jg1946frequency}.
Specifically, authors in \citep{SLIM} defined a unified embedding space where positive links between two network nodes result in close proximity in terms of their distance in a latent space, regarded as the ``sociotope''. In contrast, negative links between a network dyad result in positioning the corresponding nodes far away in terms of their latent distance in the sociotope. While such a design choice holds promise for modeling and accurately visualizing friendship and animosity in social networks, it does not directly extend to signed biological networks, and more specifically to signed protein-protein interaction networks (\textsc{SPPI}), but rather requires additional modeling design steps.

In this study, we propose the Signed Two Space Proximity Model (S$2$-SPM), the first study that formulates an archetypal-based signed network to model protein interactions.
The proposed method contributes to the existing research in the field in the following key aspects: (i) S$2$-SPM outperforms all compared baselines in terms of signed link prediction
    across three real-world PPI networks by %$2.1\%$ on average in AUC-ROC score and by 
    $4.3\%$ on average in F1 score with regards to the best competitor,
    (ii) S$2$-SPM is supported by an enrichment analysis based on the Gene Ontology (GO) terms, clarifying the biological relevance of the identified archetypes. This analysis statistically confirms the validity of the obtained representations and enables potential explainability aspects that can be crucial for the biomedical research community,
    (iii) Extensive visualizations of the obtained latent structures and archetypes highlight the effectiveness of the proposed S$2$-SPM in discovering and capturing latent structures present in \textsc{SPPI} networks,
    (iv) The consistency and robustness of the extracted structures and archetypes via S$2$-SPM is confirmed through informative measures, such as the Bayesian Normalized Mutual Information score. 

%All relevant implementations, including the proposed S$2$-SPM and the evaluation process we follow, are publicly available at \url{https://github.com/Nicknakis/S2SPM}.
%In the next sections, we provide analytical formulations and explanations of the materials and methods used to define, experimentally test, and evaluate the proposed method, followed by a thorough presentation and discussion of the obtained findings.
